NeuraCrypt: Hiding Private Health Data via Random Neural Networks for Public Training

Balancing the needs of data privacy and predictive utility is a central challenge for machine learning in healthcare. In particular, privacy concerns have led to a dearth of public datasets, complicated the construction of multi-hospital cohorts and limited the utilization of external machine learning resources. To remedy this, new methods are required to enable data owners, such as hospitals, to share their datasets publicly, while preserving both patient privacy and modeling utility. We propose NeuraCrypt, a private encoding scheme based on random deep neural networks. NeuraCrypt encodes raw patient data using a randomly constructed neural network known only to the data-owner, and publishes both the encoded data and associated labels publicly. From a theoretical perspective, we demonstrate that sampling from a sufficiently rich family of encoding functions offers a well-defined and meaningful notion of privacy against a computationally unbounded adversary with full knowledge of the underlying data-distribution. We propose to approximate this family of encoding functions through random deep neural networks. Empirically, we demonstrate the robustness of our encoding to a suite of adversarial attacks and show that NeuraCrypt achieves competitive accuracy to non-private baselines on a variety of x-ray tasks. Moreover, we demonstrate that multiple hospitals, using independent private encoders, can collaborate to train improved x-ray models. Finally, we release a challenge dataset to encourage the development of new attacks on NeuraCrypt.

==> checklist.tex <==
\newpage
\section{Check list}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work? \answerYes{} [We precisely described a threat model under which our scheme would offer security benefits. We mentioned in the paper that our scheme cannot protect the privacy under general privacy threat models, e.g., parallel data attack.]
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} [We include a discussion of this in the appendix]
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} [We fully described the assumption (here the privacy threat model) in Section~3 as ``Threat model" and in Section~4 as definition of ``Eve (adversary)".]
	\item Did you include complete proofs of all theoretical results? \answerYes{} [We included the complete proof of all theoretical parts the appendix]
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{[This is included in our code release, which is linked in the appendix.]}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} [This is also shown in our code release]
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} [Please refer to Table~1 and Table~2.]
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} [We describe the runtime of our experiments in the appendix.]
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} [We cited the datasets and ML architectures that we used in our experiments in Section~5. ]
  \item Did you mention the license of the assets?
    \answerYes{} [This is information is included in our appendix]
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} [We provide a link to all our code in the appendix.]
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> formulation.tex <==

%\subsection{Problem formulation}

The mathematical derivations used rely on both stochastic (random) and deterministic variables. The function $\Pr[\mathbf{x}=x]$ shows the probability of random variable $\mathbf{x}$ taking value $x$. We denote the set of all samples by $\mathcal{X}$. Each sample is labeled via a function $L:\mathcal{X} \rightarrow \mathcal{Y}$. Thus, we say that $L(x)$ is the label of sample $x$. For example, $\mathcal{X}$ could be the set of all chest X-ray images and $\mathcal{Y}$ a set of medical diagnosis, e.g., Normal, Edema, Pneumothorax, etc. 

In our setting, we consider $D$ data owners, e.g. hospitals, which intend to contribute their data to train an ML model while protecting privacy of their data. Each data owner $d \in \{1,\ldots,D\}$ has a subset of samples, denoted by $\{{x}_1,\dots,{x}_{|\mathcal{X}_d|}\} = \mathcal{X}^d \subseteq \mathcal{X}$, which is drawn from $\mathcal{X}$ according to some distribution $\Pr [\bm{x_1}=x_1,\ldots, \bm{x_{|\mathcal{X}^d|}}=x_{|\mathcal{X}^d|}]$.\vnote{Does the encryption algorithm need to know this distribution? Do we assume anything about this distribution, e.g. large enough entropy, for security?}\hnote{The privacy analysis requires the distribution for precisely measuring the privacy offered by a set of transforms. Without any information about the distribution, the analysis would be similar to k-anonymity. When we have distribution, all possible measures of privacy can be used for a family of transforms , e.g., guesswork analysis, MSE, etc.} The data owner also knows the labels $L(x)$, for every $x \in \mathcal{X}^d$. To preserve privacy, instead of transmitting the original data, each data owner will first apply some transformation $T^d: \mathcal{X} \rightarrow \mathcal{Z}$ on the data. This transformation is chosen from a family of possible transformations $\mathcal{F} \subseteq \mathcal{Z}^\mathcal{X}$ according to some distribution $\Pr [\bm{T^d} = T]$. Each data owner then transmits $(T^d(x),L(x))$ for every $x \in \mathcal{X}^d$ to the host of the ML model. 

The learnability goal is for the host of the ML model to be able to train his model to learn a mapping $\ML:\mathcal{Z}\rightarrow\mathcal{Y}$ such that $\ML(T^d(x))=L(x)$ with high probability, for every $d\in\{1,\dots,D\}$ and $x\in\mathcal{X}$.

% Let $\mathcal{X}=\{{x}_1,\dots,{x}_u\}$ be the set of all possible samples and $\{y_1,\dots,y_u\}$ be the set of their corresponding labels, where $y_i=L({x}_i)\in\mathcal{Y}$ is the label of sample ${x}_i$, $i\in\{1,\dots,u\}$. Here, $\mathcal{Y}=\{1,\dots,C\}$ is the set of all possible labels and $C$ is the number of classes (different labels). For example, consider $\mathcal{X}$ as the set of all possible chest X-ray images. Then, ${x}_i\in\mathcal{X}$ is a chest X-ray image, and $y_i$ can be a medical diagnosis among $C$ different possibilities e.g., Normal, Edema, etc.

% Consider $D$ data owners, e.g., $D$ hospitals, intend to safely contribute their data to train an ML model. Each data owner has a subset of samples $\{{x}_1,\dots,{x}_{|\mathcal{X}_d|}\}=\mathcal{X}_d\subseteq\mathcal{X}$, $d\in\{1,\dots,D\}$, and their labels $L({x})$, for every $x\in\mathcal{X}_d$. Each data owner with index $d\in\{1,\dots,D\}$ chooses an encoding transform $T^d:\mathcal{X}\rightarrow\mathcal{Z}$ from a set of possible encoding transforms $F=\{T_1,\dots,T_d\}$ according to distribution $P[\bm{T^d}=T]=P_{\{T,d\}}$, and then transmits $[T_d({x}),L({x})]$ for every  $x\in\mathcal{X}_d$ to the host of the ML model. We assume the samples at the data owner with index $d\in\{1,\dots,D\}$ are randomly drawn according to probability distribution \textcolor{red}{[joint distribution here]}. \vnote{Does the encryption algorithm need to know this distribution? Do we assume anything about this distribution, e.g. large enough entropy, for security?}

% The learn-ability goal is to be able to classify the samples in $\mathcal{Z}$, using a collection of labeled encoded data from one or more data owner(s). In other words, our goal is to be able to train an ML model to learn a mapping $\ML:\mathcal{Z}\rightarrow\mathcal{Y}$ such that $\ML(T_d(x))=L(x)$, for every $d\in\{1,\dots,D\}$ and $x\in\mathcal{X}$,
% with a high probability.

\paragraph{Threat model} We consider a computationally unbounded adversary which has full knowledge about the set of samples $\mathcal{X}$ and the labeling function $L: \mathcal{X} \rightarrow \mathcal{Y}$. The adversary observes all communications between the $D$ data owners and the host of the ML model and thus knows $(T^d({x}),L({x}))$, for every ${x}\in\mathcal{X}^d$ and $d\in\{1,\dots,D\}$. Moreover, because we do not have control over the classifying capabilities of the adversary, we assume the worst case in which the adversary is able to classify perfectly, i.e. we assume the adversary knows $(T^d({x}),L({x}))$, for every ${x}\in\mathcal{X}$ and $d\in\{1,\dots,D\}$. The goal of the adversary is to identify information, beyond their labels, about original samples in $\mathcal{X}^d$ from any of the $D$ data owners. \rnote{We should discuss this.} Since the data owners perform the encoding procedure independently from each other, we analyze their privacy individually. \vnote{Perfect identification of the input x-ray may not be necessary to identify sufficiently many relevant features, enough to leak PII. e.g., anyone can be identified using just 33 carefully chosen bits \url{https://33bits.wordpress.com/about/}. In our specific case, even if no adversary can reconstruct an entire x-ray image, she may be able to tell a number of relevant features of a particular image labeled, e.g., ``edema'' such as whether the person was male/female, black/white and tall/short. The key question is: do you think the method is also secure in a stronger sense where such feature reconstruction is not possible significantly better than obvious guessing using a-priori probabilities?}\hnote{I understand your point about the case that an attacker does not uniquely know the plaintext but can approximate an area around the plaintext which includes more than one chest x-rays. Then, if they share some features, attacker learns something about the plaintext. It depends on our definition of privacy then. I think our approach is close to K-anonymity which can possibly leak information about features.}\vnote{That's exactly right. $K$-anonymity is known to have significant weaknesses, e.g., \url{https://en.wikipedia.org/wiki/K-anonymity\#Possible_attacks.} and we should be careful to address it.}\hnote{Yes, I agree. I furhter discussed this with Muriel and Rafael. We show Eve with unlimited computational power and all her knowledge can obtain a list of possible values for each hospital data. Now, if no information is given about the distribution of samples, the type of privacy guarantees is close to K-anonymity without specific guarantees on feature privacy. If the distribution of samples are given, different kinds of privacy measurement can be done. For example, in that case we can do entropy analysis and find how many bits are revealed.}



% \paragraph{Threat model} We consider a computationally unbounded
% adversary that has access to the labeled encoded dataset of all data owners, i.e., $[T_d({x}),L({x})]$, for every ${x}\in\mathcal{X}_d$ and $d\in\{1,\dots,D\}$. We also assume the adversary has full knowledge of the sample space $\mathcal{X}$ with labels and the transform space $\mathcal{F}$. Moreover, because we do not have control over what classifier the adversary has, we assume the worst case in which Eve is able to classify perfectly, i.e., the adversary has $[T_d({x}),L({x})]$, for every ${x}\in\mathcal{X}$ and $d\in\{1,\dots,D\}$. The goal of the adversary is to identify one of the original messages. Since the data owners do the encoding procedure independently, we analyze their privacy individually in this paper. We note that the transforms in $\mathcal{F}$ can be reversible. Thus an adversary that finds $T_d$, $d\in\{1,\dots,D\}$, can identify $\mathcal{X}_d$ with no uncertainty. \vnote{Perfect identification of the input x-ray may not be necessary to identify sufficiently many relevant features, enough to leak PII. e.g., anyone can be identified using just 33 carefully chosen bits \url{https://33bits.wordpress.com/about/}. In our specific case, even if no adversary can reconstruct an entire x-ray image, she may be able to tell a number of relevant features of a particular image labeled, e.g., ``edema'' such as whether the person was male/female, black/white and tall/short. The key question is: do you think the method is also secure in a stronger sense where such feature reconstruction is not possible significantly better than obvious guessing using a-priori probabilities?}\hnote{I understand your point about the case that an attacker does not uniquely know the plaintext but can approximate an area around the plaintext which includes more than one chest x-rays. Then, if they share some features, attacker learns something about the plaintext. It depends on our definition of privacy then. I think our approach is close to K-anonymity which can possibly leak information about features.}\vnote{That's exactly right. $K$-anonymity is known to have significant weaknesses, e.g., \url{https://en.wikipedia.org/wiki/K-anonymity\#Possible_attacks.} and we should be careful to address it.}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/AliceBobEve.pdf}
    \caption{Alice (hospital) has a set of labeled samples. She encodes the samples and transmits the labeled encoded data to Bob (host of ML model). Eve (eavesdropper) observes Alice's transmission to Bob and, using her side information, attempts to identify information about Alice's raw data.}
    \label{fig:alice-bob-eve}
\end{figure}


==> notes/backup_of_privacy.tex <==
In this section, we present a detailed analysis of the threat model in Section \ref{sec: formulation}. 
Through this section, the space set of original samples, encoded samples, labels, and encoders are denoted with $\mathcal{X}$, $\mathcal{Z}$, $\mathcal{Y}$, and $\mathcal{F}\subseteq \mathcal{Z}^\mathcal{X}$ respectively. Without loss of generality, we consider $x_i \prec x_j$ when $i<j$ for some complete order $\preceq$ on $\mathcal{X}$. As each data-owner acts independently, we perform our analysis individually. Thus, we consider the following model with three participants, see also Figure~\ref{fig:alice-bob-eve}:

\begin{itemize}
    \item \textbf{Alice (data-owner):} Alice has a private subset of samples $X_A \subseteq \mathcal{X}$ which is drawn from a distribution $\Pr [\bm{X_A}=X_A]$. Alice samples an encoder $T_A$ from $\mathcal{F}$ according to a distribution $\Pr [\bm{T_A} = T]$, and then transmits $\{(T_A(x),L(x))\}_{x\in\ X_A}$ to Bob.
    
    \item \textbf{Bob (model host):} Bob receives $\{(T_A(x),L(x))\}_{x\in\ X_A}$, and then estimates distribution $\Pr[\bm{L(x)}=y|\bm{T(x)}=z]$ for every $x\in\mathcal{X}$.
    \item \textbf{Eve (eavesdropper):} Eve knows $\{(T_A(x),L(x))\}_{x\in\ X_A}$, $\{(x,L(x))\}_{x\in\ \mathcal{X}}$, and $\mathcal{F}$. Since Eve can also train a classifier, we consider the worst case in which she is able to perfectly classify Alice's encoded samples and thus knows $\{(T_A(x),L(x))\}_{x\in\ \mathcal{X}}$.
\end{itemize}

In our theoretical analysis, we consider only bijective encoders and thus, without loss of generality, we assume that $\mathcal{Z}=\mathcal{X}$ and $\mathcal{F}\subseteq \Sym (\mathcal{X}) = \{T:\mathcal{X}\rightarrow \mathcal{X}: \text{$T$ is bijection} \}$. 
We occasionally represent the encoder $T$ by a vector with size $|\mathcal{X}|$ whose $i$-th element is $T(x_i)$. Next we define the \textit{label configuration (LC)} and \textit{LC-anonymity list}. As we will see, these notions capture Eve's uncertainty about Alice's private samples $X_A$. 

\begin{definition}[Label Configuration] The original label configuration, denoted as $\LC(\mathcal{X})$, is a vector whose $i$-th elements is $L(x_i)$. The label configuration of an encoder $T$, denoted as $\LC(T)$, is a permutation of $\LC(\mathcal{X})$ according to $T$.
%\vnote{How does this vector depend on $T$?} 
\end{definition}


\begin{definition}[LC-Anonymity List] Given a family of encoders $\mathcal{F}$, the LC-anonymity list of an encoder $T \in \mathcal{F}$ is defined as $\mathcal{F}_{T} = \{T' \in \mathcal{F}: \LC(T')=\LC(T) \}.$
\end{definition}
The LC-anonymity lists partition $\mathcal{F}$ into different equivalence classes (see Figure~\ref{fig:EveandLCAnonimity}).

%The following example should help clarifying our notation.

% \begin{proposition}
% If Alice chooses $T\in \mathcal{F}$ uniformly at random, then the probability of Eve guessing $T$ correctly is $1/{|\mathcal{F}_{T_A}|}$.
% \end{proposition}

\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{Figures/LC_configuration2.pdf}
    \caption{Eve receives Alice's encoded data, and using her side information, selects the cluster of encoders (LC-anonymity list) with the same LC as Alice's data. Rows in a cluster show different encoders (represented by vectors), and each cluster is marked with a different color. Eve cannot distinguish among encoders within one cluster, and the best she can do is to identify all possible values for Alice's raw data corresponding to each of the encoders within the LC-anonymity list.}
    \label{fig:EveandLCAnonimity}
\end{figure}

\begin{example} \label{sec:example1}
Let $\mathcal{X} = \{1,..., 16\}$, where $1\preceq 2\preceq\dots,\preceq 16$, $\mathcal{Y}=\{-,+\}$, and $\mathcal{F}=\Sym (\mathcal{X})$. Let $\LC(\mathcal{X})=(++--++----------)$. \vnote{This is hard to read. Easier if the numbers are given along with the labels.} Assume Alice chooses $T_A=(12,2,11,4,6,8,16,15,13,7,9,5,3,14,1,10)$, 
and her data is $X_A=\{2,5,7, 10,15\}$. Thus, she sends $\{(2,+),(6,+),(16,-),(7,-),(1,-)\}$ to Bob. According to the threat model, Eve knows $\LC(T_A)=(-+---+-+---+----)$. Although $|\mathcal{F}|=16! \approx 10^{13}$, since Eve knows $\LC(T_A)$, it follows that Alice's encoder is in the set $\mathcal{F}_{T_A}$ with cardinality $4!12! \approx 10^{10}$. Thus, if Alice had chosen $T_A$ uniformly at random from $\mathcal{F}$, then the probability of Eve guessing $T_A$ correctly would be approximately ${1}/{10^{10}}$. Eve, however, is interested in learning $X_A$. But because $T_A$ is uniform over all permutations, it can be shown that she cannot learn anything about $X_A$.
\end{example}

As illustrated in the example above, if Alice chooses $T_A$ uniformly from $\Sym(\mathcal{X})$, she obtains perfect privacy. This, however, completely destroys the structure of $X_A$ making Bob's learning task more difficult. \rnote{How can we say this better? From my own notion of learning, this would make Bob's learning impossible, or equivalent to memorization.} \vnote{That's exactly right. In other words, unless you see a sample from the encoded dataset, there is no chance you can predict its label better than than a-priori probability, i.e. in the example, $\approx$ 4/16 for + and $\approx$ 12/16 for -.} In Theorem \ref{theorem: optimal scheme}, we show that there exist schemes which are perfectly private, while still preserving the structure of $X_A$. We begin by investigating the privacy of general families $\mathcal{F} \subseteq \Sym(\mathcal{X})$.

We begin by characterizing the set of possible values for $X_A$, given Eve's observations.
%Let define $\mathcal{X}^y \triangleq \{x_i \in \mathcal{X}: y_i = y \}$ and $X_A^y \triangleq \{x_i \in X_A: y_i = y \}$, for every $y \in \mathcal{Y}$. Eve, only by looking at the label $y$ of Alice's encoded sample $T(x)$, $x\in X$, identifies that $x$ must be in $\mathcal{X}^{y}$. If the samples in $X$ were chosen uniformly and independently at random from $\mathcal{X}$, Eve would be able to correctly guess a sample in $X$ with label $y\in\mathcal{Y}$ with probability $|X^{y}|/|\mathcal{X}^y|$. This probability is a lower-bound on the actual probability of Eve guessing a sample with label $y$ correctly as Eve did not use $\LC(T)$. Next, we consider the general family of encoders $\mathcal{F}$.
\begin{proposition}
The set of possible values for Alice's dataset is given by 
\[ \Pos(X_A) \triangleq \{\Bar{X} \in \mathcal{X}^{|X_A|} :  \exists T \in \mathcal{F}_{T_A} \text{ with } T(\Bar{X}) = T_A(X_A)\} .\]
\end{proposition}

The next lemma characterizes all that Eve learns given her observations of what Alice sends to Bob, and thus characterizes the privacy loss because of the choice of $\mathcal{F}$.


\begin{lemma} \label{lemma:probAlice}
Let $\bm{X_A}$ be the random variable for Alice's private samples and $\bm{T_A}$ be the random variable for Alice's encoder. Then, $\Pr[\bm{X_A}= \Bar{X} , \bm{T_A} = T \mid \bm{T _A({X_A})}=Z,\; \bm{\LC(T_A)}=\LC]$ is proportional to $\mathbbm{1} (T(\Bar{X})=Z) \cdot \mathbbm{1}(\LC(T)=\LC) \cdot \Pr[\bm{{X}_A}=\Bar{X}] \cdot\Pr{[ \bm{T_A} = T]}$. Here, $\mathbbm{1}(C)$ is $1$ if $C$ is true, and $0$ otherwise.
\end{lemma}

Since Lemma~\ref{lemma:probAlice} fully characterizes how much Eve learns about Alice's private samples and the encoder $T_A$, any privacy metric, be it a mutual information \citep{Shannon48}, a mean squared error \citep{}, or a guessing measure \citep{}, can be computed from Lemma \ref{lemma:probAlice}. For example, if Eve is interested solely on Alice's private samples and not the encoder, the following proposition is of use.

\begin{proposition} \label{prop1:AlicProb}
Let $\bm{X_A}$ be the random variable for Alice's private samples and $\bm{T_A}$ be the random variable for Alice's encoder. Then,
\begin{equation*}
    \begin{split}
        \Pr[\bm{X_A} &= \Bar{X} \mid \bm{T_A ({X}_A)}=Z,\; \bm{\LC(T_A)}=\LC]\propto \sum_{\{T:\LC(T)=L,T(\Bar{X})=Z\}}\Pr[\bm{{X}_A}=\Bar{X}]\Pr{[ \bm{T_A} = T]}
    \end{split}
\end{equation*}
and
\[ \Pr[x \in \bm{X_A}] = \sum_{\Bar{X} \ni x}  \Pr[\bm{X_A} = \Bar{X} \mid \bm{T_A({X_A})}=Z,\; \bm{\LC(T_A)}=L] \]
\end{proposition}

%\bigskip
%\hline
%\bigskip

%\begin{theorem}
%\[\Pr[\bm{\mathcal{X}_A} = \Bar{x} , \bm{T_A} = T \mid \bm{T_A (\mathcal{X}_A)} = m , \Shape(\bm{T_A})=s] \] 
%\[\propto \]
%\[\mathbbm{1} [T(\Bar{x})=m] \cdot \mathbbm{1} [\Shape(T)=s] \cdot \Pr[\bm{\mathcal{X}_A}=T^{-1}(m)] \cdot \Pr[\bm{T_A}=T] \]
%\end{theorem}

%\begin{proof}
%\[\Pr[\bm{\mathcal{X}_A} = \Bar{x} , \bm{T_A} = T \mid \bm{T_A (\mathcal{X}_A)} = m , \Shape(\bm{T_A})=s] \] 
%\[= \]
%\[ \Pr[\bm{\mathcal{X}_A} = \Bar{x} \mid \bm{T_A} = T , \bm{T_A (\mathcal{X}_A)} = m , \Shape(\bm{T_A})=s] \cdot \Pr[\bm{T_A} = T \mid \bm{T_A (\mathcal{X}_A)} = m , \Shape(\bm{T_A})=s] \]
%\[= \]
%\[ {\color{red}\mathbbm{1} [T(\Bar{x})=m]} \cdot \Pr[\bm{T_A} = T \mid \bm{T_A (\mathcal{X}_A)} = m , \Shape(\bm{T_A})=s]\]
%\[\propto \]
%\[\mathbbm{1} [T(\Bar{x})=m] \cdot \Pr[\bm{T_A (\mathcal{X}_A)} = m \mid  \bm{T_A} = T , \Shape(\bm{T_A})=s] \cdot \Pr[\bm{T_A} = T \mid \Shape(\bm{T_A})=s] \]
%\[= \]
%\[\mathbbm{1} [T(\Bar{x})=m] \cdot \Pr[\bm{\mathcal{X}_A} = T^{-1}(m)] \cdot \Pr[\bm{T_A} = T \mid \Shape(\bm{T_A})=s] \]
%\[\propto \]
%\[\mathbbm{1} [T(\Bar{x})=m] \cdot \Pr[\bm{\mathcal{X}_A} = T^{-1}(m)] \cdot \Pr[\Shape(\bm{T_A})=s \mid \bm{T_A} = T] \cdot \Pr[\bm{T_A} = T] \]
%\[=\]
%\[\mathbbm{1} [T(\Bar{x})=m] \cdot \mathbbm{1} [\Shape(T)=s] \cdot \Pr[\bm{\mathcal{X}_A}=T^{-1}(m)] \cdot \Pr[\bm{T_A}=T] \]
%\end{proof}
%\bigskip
%\hline
%\bigskip



%In general, the probability distribution of $\mathcal{X}_A$ and $T_A$ induce a probability distribution on $\Pos(\mathcal{X}_A, L, \mathcal{F})$, that enables us to do a variety of privacy analysis, see Figure~\ref{fig:EveandPrivacy}. 



% \begin{proposition}\label{prop2:AlicProb} 
% $\Pr[x \in X_A] = \sum_{x \in \Bar{X} \in \Pos(X_A)} \Pr[\bm{X_A} = \Bar{X} \mid \bm{T_A({X_A})}=Z,\; \bm{\LC(T_A)}=L]$
% \end{proposition}

\begin{example}
Let $\mathcal{X}=\{1,2,3,4,5\}$, $X_A = \{2,3,4\}$, $\LC(\mathcal{X}) =(++---)$, and $\mathcal{F}=\{T_1,\dots,T_6\}$ given below. Suppose $T_A = T_1$. Then, Alice transmits $\{(1,+),(4,-),(5,-)\}$. Eve knows $\LC(T_A) =(++---)$, and thus knows $\mathcal{F}_{T_A}$ as well:
\begin{equation*}
\mathcal{F}=\begin{cases}
T_1:&(2,1,5,4,3)\\ 
T_2:&(2,1,3,5,4)\\ 
T_3:&(1,2,3,5,4)\\ 
T_4:&(4,3,1,2,5)\\ 
T_5:&(3,4,2,1,5)\\ 
T_6:&(5,2,4,3,1)
\end{cases},\quad
\mathcal{F}_{T_A}=\begin{cases}
T_1:&(2,1,5,4,3)\\ 
T_2:&(2,1,3,5,4)\\ 
T_3:&(1,2,3,5,4)\\ 
\end{cases}.
\end{equation*}
As a result, $\Pos (X_A) = \{ (2,4,3), (2,5,4), (1,5,4) \}$. Thus, Eve knows that $4 \in X_A$ independent distribution of $X_A$. If we assume uniform distributions for $T_A$ and $X_A$, then, by Lemma \ref{lemma:probAlice}, we obtain a uniform distribution on $\Pos (X_A)$ and from Proposition \ref{prop1:AlicProb} we can compute $\Pr[1 \in X_A]={1}/{3}$ and $\Pr[2 \in X_A] = {2}/{3}$. If instead we assume uniform $T_A$ and $\Pr[X_A=\{2,3,4\}] = 0.1$, $\Pr[X_A=\{2,5,4\}] = 0.1$, and $\Pr[X_A=\{1,5,4\}] = 0.4$, then $\Pr[1 \in X_A] = {2}/{3}$ and $\Pr[2 \in X_A] = {1}/{3}$. A more detailed version of this example is given in the Appendix.
\label{exmaple2:extensive}
\end{example}

We now describe an \textit{optimal} scheme for both privacy and learnability. 

\begin{theorem} \label{theorem: optimal scheme}
Let $\mathcal{X}^y = \{x \in \mathcal{X}: L(x) = y \}$. Then, sampling $T_A$ uniformly from the family $\mathcal{F}_0 = \{T \in \Sym (\mathcal{X}) : T(\mathcal{X}^y) = \mathcal{X}^y \quad \forall y \in \mathcal{Y} \}$ is optimal for both privacy and learnability.
\end{theorem}

Although Theorem \ref{theorem: optimal scheme} shows the existence of an optimal scheme, Alice has no way of determining it under our threat model, since it would require knowledge of the full labeling of $\mathcal{X}$. In practice, however, Alice does have some knowledge of the labeling of $\mathcal{X}$ \vnote{But in our design, the transformation is task-agnostic and so Alice does not use any such knowledge (beyond annotating the encoded samples with the right labels).} and, thus, the theorem serves as a guide on what properties Alice might want from the family of encoders $\mathcal{F}$.

In constructing $\mathcal{F}$, an important question is: what kind of operations can increase the privacy of $\mathcal{F}$? In our next proposition, we show that adding arbitrary functions to $\mathcal{F}$ might actually worsen privacy.

% Next, we show how function composition results in family of encoders with improved privacy, supporting the \name architecture which is based on composition of a sequence of functions realized by convolutional layers. First, in Proposition~\ref{prop:addingcanhurt}, we show adding an encoder to $\mathcal{F}$ can actually make it less safe.

\begin{proposition} \label{prop:addingcanhurt} Let $\mathcal{F}, \mathcal{F}' \in \Sym (\mathcal{X})$ be two families of encoders such that $\mathcal{F} \subseteq \mathcal{F}'$. Then, it is not generally true that $\mathcal{F}'$ is more private than $\mathcal{F}$.
\end{proposition}

Thus, adding encoders to $\mathcal{F}$ can potentially make it less private. However, as we now show, composing families of functions can never decrease privacy, but can potentially increase it.

\begin{theorem} \label{theorem:compositiondoesnothusrt}
Let $\mathcal{F}, \mathcal{F}' \in \Sym (\mathcal{X})$ and $\mathcal{F}' \circ \mathcal{F} = \{ T' \circ T : T' \in \mathcal{F}', T \in \mathcal{F} \}$. Then, $\mathcal{F}' \circ \mathcal{F}$ is no less private than $\mathcal{F}$.
\end{theorem}

Theorem \ref{theorem:compositiondoesnothusrt} shows that composing families of encoders cannot reduce the privacy. Indeed, as we show in the following example, in can potentially increase it.

\begin{example}
\label{ex:compositionhelp}
Let $\mathcal{X}=\{1,2,3,4,5\}$, $\LC(\mathcal{X})=(++---)$. The sets of encoders $\mathcal{F}$, $\mathcal{F}'$, and  $\mathcal{F}\circ\mathcal{F}'$, along with the label configuration for each encoder, are given:

\begin{minipage}[c]{0.45\linewidth}
     \begin{equation*}
        \mathcal{F}=\begin{cases}
        T_1:&(1,2,3,4,5),(++---)\\ 
        T_2:&(2,1,3,5,4),(++---)\\ 
        T_3:&(1,2,5,4,3),(++---)\\ 
        T_4:&(1,3,2,4,5),(+-+--)\\ 
        T_5:&(1,5,2,3,4),(+-+--)
        \end{cases}
    \end{equation*}
        \begin{equation*}
        \mathcal{F'}=\begin{cases}
        T'_1:&(1,2,3,4,5),(++---)\\ 
        T_2:&(3,2,1,4,5),(-++--) 
        \end{cases}
    \end{equation*}
\end{minipage}
\begin{minipage}[c]{0.52\linewidth}
    \begin{equation*}
    \mathcal{F'}\circ\mathcal{F}=\begin{cases}
        T'_1\circ T_1:&(1,2,3,4,5),(++---)\\ 
        T'_1\circ T_2:&(2,1,3,5,4),(++---)\\ 
        T'_1\circ T_3:&(1,2,5,4,3),(++---)\\ 
        T'_1\circ T_4:&(1,3,2,4,5),(+-+--)\\ 
        T'_1\circ T_5:&(1,5,2,3,4),(+-+--)\\ 
        T'_2\circ T_1:&(3,2,1,4,5),(-++--)\\ 
        T'_2\circ T_2:&(3,1,2,5,4),(-++--)\\ 
        T'_2\circ    T_3:&(5,2,1,4,3),(-++--)\\ 
        T'_2\circ T_4:&(2,3,1,4,5),(+-+--)\\ 
        T'_2\circ          T_5:&(2,5,1,3,4),(+-+--) 
        \end{cases}
    \end{equation*}
\end{minipage}

Here, $\mathcal{F}$ has two LC-anonymity lists, with cardinality $2$ and $3$, and $\mathcal{F}'\circ\mathcal{F}$ has three LC-anonymity lists with cardinality $3$, $3$, and $4$. Thus, it offers more ambiguity (better privacy) as its LC-anonymity lists have higher minimum cardinality compared to $\mathcal{F}$ alone.
\end{example}

In fact, composition permutes the label configuration of encoders in $\mathcal{F}$ according to different encoders in $\mathcal{F}'$. This can possibly generate more LC-anonymity lists, but minimum cardinality of LC-anonymity lists is at least equal to the one for  $\mathcal{F}$. Thus, composition can never worsen the privacy, and can possibly improve it as we saw in the example. This motivates our \name approach since the layers of the neural network are essentially composed with each other.

[some connecting sentences to \name here]
